Improved Round-by-round Soundness IOPs via Reed-Muller Codes

We give an IOPP (interactive oracle proof of proximity) for trivariate Reed-Muller codes that achieves the best known query complexity in some range of security parameters. Specifically, for degree $d$ and security parameter $\lambda\leq \frac{\log^2 d}{\log\log d}$ , our IOPP has $2^{-\lambda}$ round-by-round soundness, $O(\lambda)$ queries, $O(\log\log d)$ rounds and $O(d)$ length. This improves upon the FRI [Ben-Sasson, Bentov, Horesh, Riabzev, ICALP 2018] and the STIR [Arnon, Chiesa, Fenzi, Yogev, Crypto 2024] IOPPs for Reed-Solomon codes, that have larger query and round complexity standing at $O(\lambda \log d)$ and $O(\log d+\lambda\log\log d)$ respectively. We use our IOPP to give an IOP for the NP-complete language Rank-1-Constraint-Satisfaction with the same parameters. Our construction is based on the line versus point test in the low-soundness regime. Compared to the axis parallel test (which is used in all prior works), the general affine lines test has improved soundness, which is the main source of our improved soundness. Using this test involves several complications, most significantly that projection to affine lines does not preserve individual degrees, and we show how to overcome these difficulties. En route, we extend some existing machinery to more general settings. Specifically, we give proximity generators for Reed-Muller codes, show a more systematic way of handling ``side conditions'' in IOP constructions, and generalize the compiling procedure of [Arnon, Chiesa, Fenzi, Yogev, Crypto 2024] to general codes.

==> line_plane/line_vs_point.tex <==
\subsection{The Line versus Point Test}

In this section we discuss the line versus point test. For our applications we will have to show that it works even when the lines table is randomized, and that in the non-trivial passing case, one can conclude a degree $d$ function that agrees on average with the randomized lines table. 

By a randomized lines table of degree $d$, $T$, we mean that $T$ has entries indexed by affine lines $L \subseteq \Ff_q^m$, and for each affine line $L$, $T[L]$ is a random degree $d$ function from $L \to \Ff_{q'}$. 

\begin{theorem} \label{thm: line vs point randomized agree}
    Let $Q: \Ff_q^m \to \Ff_{q'}$ be a points table and let $T$ is a randomized lines table of degree $d$ such that
    \[
    \Pr_{L, T[L], x \in L}[T[L](x) = Q(x)] = \eps \geq 20\cdot \left(\frac{d}{q}\right)^{\tau}.
    \]
    Then there exists a degree $d$ function $H: \Ff_q^m \to \Ff_{q'}$ satisfying,
    \[
    \Pr_{L, T[L]}[T[L] = H|_L] \geq \frac{\eps}{5}.
    \]
\end{theorem}

Towards the proof of \cref{thm: line vs point randomized agree}, we will first show a list decoding version of \cref{thm: line vs point points agree}. This variant is obtained using standard techniques. 
\begin{theorem} \label{thm: line vs point list decode}
     Suppose the setup of \cref{thm: line vs point randomized agree}. Then there is a list of degree $d$ functions $\{f_1,\ldots, f_M\}$ such that $M \leq O(\eps^{-2})$,
     \[
     \Pr_{x \in \Ff_q^m, L \ni x}[T[L](x) = Q(x) \land Q(x) \notin \{f_i(x)\}_{i=1}^M] \leq \frac{\eps}{2},
     \]
     and for each $i \in M$,
     \[
     \Pr_{x \in \Ff_q^m}[Q(x) = F_i(x)] \geq \frac{\eps}{4}.
     \]
\end{theorem}
\begin{proof}
      Let $\{f_1,\ldots, f_M\}$ be the list of degree $d$ polynomials that agree with $Q$ on at least $\eps/4$-fraction of the points in $\Ff_q^m$. By [LIST DECODING BOUNDS], $M \leq O(\eps^{-2})$. 
      
      We claim that $\{f_1, \ldots, f_M \}$ are the desired list of functions. Suppose for the sake of contradiction that this is not the case. That is, suppose
      \begin{equation}   \label{eq: line point assump}
      \Pr_{x \in \Ff_q^m, L \ni x}[T[L](x) = Q(x) \land Q(x) \notin \{f_i(x)\}_{i=1}^M] > \frac{\eps}{2}.
    \end{equation}

      For each $i \in [M]$, let $W_i = \{x \subseteq \Ff_q^m \; | \; Q(x) = F_i(x)\}$. Consider the randomized points table $Q'$ obtained by choosing $Q'(x)$ randomly for every $x \in \cup_{i=1}^M W_i$ and keeping $Q'(x) = Q(x)$ for all other points $x$. By a straightforward calculation, with nonzero probability $Q'$ has agreement at most $0.26\eps$ with every polynomial of degree $d$ and we fix this $Q'$ henceforth. 

      On the other hand, by Equation~\eqref{eq: line point assump}, $T$ and $Q'$ will pass with probability at least $\eps/2$ due to the points $x \notin \cup_{i=1}^M W_i$ alone, so
    \[
      \Pr_{x \in \Ff_q^m, L \ni x}[T[L](x) = Q'(x)] > \frac{\eps}{2}.
      \]
    \cref{thm: line vs point points agree} then implies that there is a degree $d$ polynomial with agreement at least 
    \[
    \frac{\eps}{2}- \left(\frac{d}{q}\right)^\tau >0.26\eps
    \]
    with $Q'$ and contradiction.
\end{proof}
We are now ready to prove \cref{thm: line vs point randomized agree}
% \begin{theorem} \label{thm: line vs point lines agree}
%     Suppose the setup of \cref{thm: line vs point randomized agree}. Then, there exists a degree $d$ function $F$ satisfying,
%     \[
%     \Pr_{L \subseteq \Ff_q^m}[T[L] = F|_L] \geq \frac{\eps}{2}.
%     \]
% \end{theorem}
\begin{proof}[Proof of \cref{thm: line vs point randomized agree}]
Let $f_1, \ldots, f_M$ be the degree $d$ functions given by Theorem~\ref{thm: line vs point list decode}. For each $i$, let $W_i = \{x \in \Ff_q^m \; | \; Q(x) = f_i(x) \}$ and let $W = \bigcup_{i=1}^k W_i$. 

For an affine line $L$ and random entry $T[L]$ let $E_i$ be the event that $T[L] = f_i|_L$. Let $E = E_1 \lor \ldots \lor E_M$. Then we can rewrite the pass probability from \cref{thm: line vs point randomized agree} as:

\begin{align}
  \Pr_{L, x \in L, T[L]}[T[L](x) = Q(x)]  &= \Pr_{L, x \in L, T[L]}[T[L](x) = Q(x) \land E \land x \in W]\\
  &+ \Pr_{L, x \in L, T[L]}[T[L](x) = Q(x) \land \overline{E} \land x \in W] \\
    &+  \Pr_{L, x \in L, T[L]}[T[L](x) = Q(x) \land x \notin W]\\
    &= \eps.
\end{align}


We will show that the first term must be non-trivial and then further dissect it. To this end, we start by upper bounding the second term and third terms from the left hand side above.

For the third term, note that by \cref{thm: line vs point list decode} we have
\[
\Pr_{L, x \in L, T[L]}[T[L](x) = Q(x) \land x \notin W] \leq \frac{\eps}{2}.
\]

For the second term we have
\begin{align*}
 \Pr_{L, x \in L, T[L]}[T[L](x) = Q(x) \land \overline{E} \land x \notin W] 
 &= \Pr_{L, x \in L, T[L]}[T[L](x) \in \{f_1(x), \ldots, f_M(x) \} \land \overline{E}] \\
 &\leq   \sum_{i=1}^M \Pr_{L, x \in L, T[L]}[T[L](x) = f_i(x) \; | \; T[L] \neq f_i|_L] \\
 &\leq M \cdot \frac{d}{q} \\
\end{align*}
In the second transition, we perform a union bound and in the third transition we use the Schwartz-Zippel lemma along with the fact that $T[L]$ and $f_i$ are distinct degree $d$ functions on the affine line $L$.

It follows that 
\[
\Pr_{L, x \in L, T[L]}\left[T[L](x) = Q(x) \land E \land x \in W \right] \geq \eps - \frac{\eps}{2} - M\cdot \frac{d}{q} \geq 0.49\eps.
\]
Performing a union bound on the above probability, we get
\begin{align*}
    \sum_{i, j = 1}^k \Pr_{L, x \in L, T[L]}\left[T[L](x) = Q(x) \land T[L] = f_i|_: \land Q(x) = f_j(x) \right]
    &\geq \Pr_{L, x \in L, T[L]}\left[T[L](x) = Q(x) \land E \land x \in W \right] \\
    &\geq \frac{9\eps}{10}
\end{align*}
Fix $i \neq j$ and consider a term in the summation above. We can bound the term by 
\[
\Pr_{L, x \in L, T[L]}\left[T[L](x) = Q(x) \land T[L] = f_i|_L \land Q(x) = f_j(x) \right] \leq \Pr_{x} \left[f_i(x) = f_j(x) \right] \leq \frac{d}{q}.
\]
It follows that 
\[
\sum_{i=1}^M \Pr_{L, x \in L, T[L]} \left[T[L](x) = Q(x) \land T[L] = f_i|_L \land Q(x) = f_j(x) \right] \geq 0.49\eps - \frac{M^2d}{q} \geq 0.48\eps
\]


For each $i$, let $F_i : G(m, 1) \xrightarrow{} [0,1]$ be the function given by $F_i[L] = \Pr_{T[L]}[T[L] = f_i|_L]$. Suppose $x$ is sampled first, and then $L \ni x$, and finally $T[L]$. We can upper bound  the probabilities in the summation as
\[
\sum_{i = 1}^M \Pr_{x}[x \in W_i] \cdot \Pr_{x \in W_i, L \ni x, T[L]}[T[L] = f_i|_L] = \sum_{i = 1}^M \Pr_{x}[x \in W_i] \E_{x \in W_i, L \ni x}[F_i(L)].
\]
Finally, because each $W_i$ consists of at least $\eps/4$-fraction of points, we have
\[
\left|\E_{P}[F_i(P)] -  \E_{x \in W_i, P \ni x}[F_i(P)]\right| \leq \frac{q^{-1/2}}{\sqrt{\eps/4}}
\]
Putting everything together, we get that
\[
\sum_{i = 1}^M \Pr_{x}\left[x \in W_i \right] \E_{P}[F_i(P)] \geq 0.48\eps - \frac{q^{-1/2}}{\sqrt{\eps/4}} \geq 0.47\eps.
\]
It follows that there exists some $i$ such that 
\[
\E_{L, T[L]}[F_i(L)] \geq 0.47\eps \cdot \left(\sum_{i = 1}^M \Pr_{x}\left[x \in W_i \right] \right)^{-1}.
\]
To conclude we note that the extra factor on the right hand side cannot be too large because the $W_i$'s have pairwise small intersections. Indeed,
\[
1 \geq \Pr_{x}\left[x \in W \right] \geq \sum_{i = 1}^M \Pr_{x}\left[x \in W_i \right] - \sum_{i \neq j} \Pr_{x} \left[x \in W_i \cap W_j \right].
\]
For fixed, $i \neq j$, $\Pr_{x} \left[x \in W_i \cap W_j \right] \leq \frac{d}{q}$. It follows that,
\[
 \sum_{i = 1}^M \Pr_{x}\left[x \in W_i \right] \leq 1 + \frac{M^2d}{q} \leq 2.
\]
As a result, for the degree $d$ function $f_i$, we have
\[
\E_{L, T[L]}[F_i(L)]  = \Pr_{L, T[L]}[T[L] = f_i|_L] \geq \frac{\eps}{5}.
\]
\end{proof}

From \cref{thm: line vs point lines agree}, we can use essentially the same proof as that of \cref{thm: line vs point list decode} to obtain a list decoding version where the agreement is with the lines table.

\begin{theorem} \label{thm: line vs point list decode lines}
     Suppose the setup of \cref{thm: line vs point points agree} with $\eps > 100(d/q)^\tau$. Then there is a list of degree $d$ functions $\{f_1,\ldots, f_M\}$ such that $M \leq O(\eps^{-2})$,
     \[
     \Pr_{x \in \Ff_q^m, L \ni x}[T[L](x) = Q(x) \land T[L] \notin \{f_i|_L\}_{i=1}^M] \leq \frac{\eps}{10},
     \]
     and for each $i \in M$, $\Pr_{L \subseteq \Ff_q^m}[T[L] = F_i|_L] \geq \eps/100$.
\end{theorem}

\begin{theorem} \label{thm: line versus line}
    Line versus Line.
\end{theorem}

% \subsubsection{The Plane versus Point Test}

% The following lemma will be the main piece of our soundness analysis.

% \begin{lemma}
%     Suppose $f: \Ff_q^m \to \Ff_q$ satisfies
%     \[
%     \agr(f, \RM[m, d]) \leq \delta.
%     \]
%     Then,
%     \[
%     \Pr_{P \subseteq \Ff_q^m}[\agr(f|_P, \RM[2,d]) \geq 2\delta] \leq \frac{1}{q^{-1/10}}.
%     \]
% \end{lemma}
% \begin{proof}
%     ...
% \end{proof}

% \begin{lemma} \label{lm: expected agreement}
% Suppose $f: \Ff_q^3 \xrightarrow[]{} \Ff_q$ satisfies 
% \[
%     \agr(f, \mathcal{F}_i) \leq \delta_i,
% \]
% where $\mathcal{F}_i = \RM[3,6\cdot \ell \cdot t]|_{f(B_i)}$ for some set of points $B_i \subseteq \Ff_q^3$. Then, for any $Q_i: \Ff_q^6 \xrightarrow[]{} \Ff_q$ satisfying, 
% \[
% Q_i(I_{t}(x_1,x_2,x_3)) = f_i(x_1, x_2, x_3),
% \]
% the following holds. 
% \begin{itemize}
%     \item Choose a point of the form $s \in \{I_{d_i}(x) \; | \; x\in \Ff_q^3\} $ uniformly at random, set $B_{i+1} = B_i \cup \{s\}$, and (arbitrarily) label the elements $b_1, \ldots, b_{\ell}$, where $\ell = |B_{i+1}|$, and $b_{\ell} = s$.
%     \item Choose a random curve $\mathcal{C}: \Ff_q \xrightarrow[]{} \Ff_q^6$ of degree $\ell$ such that $\C(\gamma_j) = b_j$ for $1 \leq j \leq \ell$. Choose a random plane $P$. Set 
%     \[
%     \mathcal{M}_i = \spa(\mathcal{C} + P).
%     \]
% \end{itemize}
% Then,
%  \[
%  \E_{\mathcal{M}_i}[\agr(Q|_{\mathcal{M}_i}, \mathcal{F}_{i+1})] \leq 10\delta_i,
%  \]
%  where 
%  \[
%  \mathcal{F}_{i+1} = \RM[3, 6\cdot \ell \cdot t^{1/2}\; | \; (b'_j, \alpha'_j)_{j=1}^{\ell+1}  ]|, \quad b'_j = (\gamma_j, 0, 0),  \quad \text{and } \alpha'_j =Q_i(b_j).
%  \]
% \end{lemma}
% \begin{proof}
%     Suppose for the sake of contradiction that this is not the case. Let $Q$ be as defined in the IOP and let $b'_j = I_{d_i}(b_j)$ for $1\leq j \leq \ell$. Let $S = \{I_{d_i}(x) \; | \; x\in \Ff_q^3\}$.

    
%     For each manifold $\M$ of the form $\mathcal{M} = \spa(\mathcal{C} + P)$, where $P \subseteq \Ff_q^{6}$ is a (linear) plane and $\mathcal{C}: \Ff_q \xrightarrow[]{} \Ff_q^6$ is a curve of $\ell$ degree satisfying,
%     \begin{align} \label{eqn: curve req}
%             \mathcal{C}(\gamma_j) &= b_j \quad \forall 1 \leq j \leq \ell-1, \\
%             \mathcal{C}(\gamma_{i+1}) &\in S,
%     \end{align}
%     let $h_{\mathcal{M}}: \Ff_q^3 \xrightarrow{} \Ff_q$ be the function in $\RM_{q,3}[6\ell t^{1/2} \; | \; \{(b_j, \alpha_j)  \}_{j=1}^{i+1}]$,
%     that is closest to $Q|_{\mathcal{M}}: \Ff_q^3 \xrightarrow[]{} \Ff_q$. By assumption,
%     \begin{equation} \label{eq: agreement in lemma}
%     \E_{\mathcal{M}}[\agr(Q|_{\mathcal{M}}, h_{\mathcal{M}})] \geq 10 \delta_i.
%     \end{equation}

%     We will now argue that there is a randomized low degree planes table that passes the plane vs. point test with $Q$ with non-trivial probability.
    
%     To this end, consider the following distribution which outputs an affine plane $P' \subseteq \Ff_q^6$ and a function $T[P']:P' \xrightarrow[]{} \Ff_q$ with degree at most $6\ell t^{1/2}$
%     \begin{itemize}
%         \item Choose a uniformly random $s \in S$.
%         \item Choose a uniformly random manifold curve $\mathcal{C}$ of degree $\ell$ satisfying \eqref{eqn: curve req} and $\mathcal{C}(\gamma_{i+1}) = s$.
%         \item Choose a uniformly random $\gamma \in \Ff_q \setminus \{\gamma_1, \ldots, \gamma_{i+1}\}$.
%         \item Output the plane $P' = C(\gamma) + P$ and the function $T[P']: \Ff_q^2 \xrightarrow[]{} \Ff_q$ given by 
%         \[T[P'](z_1, z_2) = h_{\mathcal{M}}(\gamma, z_1, z_2)
%         \]
%     \end{itemize}
%     Note that in the above distribution, the output plane $P'$ is uniformly random.
    
%     Using the above distribution, we define the randomized planes table $T$ as follows. For each plane $P$, $T[P]: P \xrightarrow{} \Ff_q$ is a bivariate function of total degree at most $6\ell t^{1/2}$, chosen uniformly at random according to the above distribution conditioned on plane $P$ being output. It follows from Equation~\eqref{eq: agreement in lemma} that this randomized planes table $T$ and $Q$ pass the planes versus point test with probability at least $C\delta$:
%     \[
%     \Pr_{P, T[P], x \in P}[T[P](x) = Q(x)] = \Pr_{\mathcal{M}, x \in \mathcal{M}}[h|_{\mathcal{M}}(x) = Q(x)] \geq 10\delta_i.
%     \]

%     By Theorem~\ref{thm: basic pvp} that there exists a function $g: \Ff_q^6 \xrightarrow[]{} \Ff_q$ of total degree at most $6\ell t^{1/2}$ such that
%     \[
%     \Pr_{P, T[P]}[g|_P = T[P]] = \E_{s, \mathcal{M} \ni s} \E_{\gamma}\left[h_{\mathcal{M}}(\gamma, z_1, z_2) = g|_{P} \right] \geq 5\delta_i.
%     \]
%     Let $\Tilde{g}: \Ff^3_q \xrightarrow[]{} \Ff_q$ be the function given by,
%     \[
%     \Tilde{g}(z_1, z_2, z_3) = g(z_1^{t^{1/2}}, z_1, z_2^{t^{1/2}}, z_2, z_3^{t^{1/2}}, z_3).
%     \]
%     We claim that $\agr(\Tilde{g}, f) \geq 5\delta_i$ and $g \in \mathcal{F}_{i}$.

%     For the first item, note that for at least $\frac{5\delta_i}{2}$-fraction of points $s$, there exists a manifold $\mathcal{M} \ni s$ such that
%     \[
%     \E_{\gamma}[h_{\mathcal{M}}(\gamma, z_1, z_2) = g|_{\mathcal{M}}(\gamma, z_1, z_2)] \geq \frac{5\delta_i}{2}.
%     \]
%     Moreover. $\deg(h_{\mathcal{M}}) \leq 6(i+1)t^{1/2}$ and $\deg(g|_{\mathcal{M}}) \leq 6(i+1)t^{1/2}$. However, by the Schwartz-Zippel Lemma, if $h|_{\mathcal{M}} \neq g|_{\mathcal{M}}$, then
%     \[
%     \Pr_{\gamma \in \Ff_q \setminus \{\gamma_1, \ldots, \gamma_{i+1} \}}[g|_{\mathcal{M}}(\gamma, z_1, z_2) = h|_{\mathcal{M}}(\gamma, z_1, z_2) ] \leq \frac{6\ell t^{1/2}}{q} + \frac{\ell}{q} < 5\delta_i. 
%     \]
%     It follows that $g_{\mathcal{M}} = h|_{\mathcal{M}}$, and in particular we have, 
%     \[
%     g(s) = g|_{\mathcal{M}}(\gamma_\ell)= h|_{\mathcal{M}}(\gamma_{\ell}) = Q(s).
%     \]
%     For each $s = (z_1^{t^{1/2}}, z_1, z_2^{t^{1/2}}, z_2, z_3^{t^{1/2}}, z_3)$, we have
%     \[
%     g(s) = \Tilde{g}(z_1, z_2, z_3) \quad \text{and} \quad Q(s) = f(z_1, z_2, z_3).
%     \]
%     Thus 
%     \[
%     \agr(\Tilde{g}, f) = \Pr_{s}[g(s) = Q(s)] \geq 5\delta_i
%     \]

%     For the second item, since there is at least one manifold $\mathcal{M}$ such that $g|_{\mathcal{M}} = h|_{\mathcal{M}}$, we have
%     \[
%     g(b_j) = g|_{\mathcal{M}}(\lambda_j) = h|_{\mathcal{M}}(\lambda_j) = \alpha_j.
%     \]
%     Moreover, since the total degree of $g$ is at most $6t^{1/2}$, it follows that $\deg(\tilde{g}) \leq 6\ell t$. Therefore $\tilde{g} \in \mathcal{F}_{i+1}$.
% \end{proof}




==> line_plane/plane_vs_point.tex <==
\subsection{Plane vs. Point}

\begin{theorem} \label{thm: basic pvp}
    Let $T$ be a randomized planes table, let $Q$ be a points table, and let the ambient space be $\Ff_q^m$. If 
    \[
    \Pr_{P, x}\left[T[P](x) = Q(x) \right] = \eps \geq \frac{1000d^{10}}{q^{1/10}},
    \]
    then there exists a degree $d$ function $h$ such that
    \[
    \Pr_{x}[h(x) = Q(x)] \geq \eps - \frac{10d^{10}}{q^{1/10}} \geq \frac{\eps}{2}.
    \]
\end{theorem}
\begin{proof}
    True by Moshkovitz-Raz analysis, or Raz-Safra analysis. Also holds if $T$ is randomized by fixing a $T$ that obtains the expected pass probability.
\end{proof}

\begin{theorem} \label{thm: list decoding pvp}
     Let $T$ be a randomized planes table, let $Q$ be a points table, and let the ambient space be $\Ff_q^m$. If 
    \[
    \Pr_{P, x}\left[T[P](x) = Q(x) \right] = \eps \geq \frac{1000d^{10}}{q^{1/10}},
    \]
    then there exists a list of $k$ degree $d$ functions, $f_1, \ldots, f_k$ with $k \leq O\left(\eps^{-2}\right)$, such that,
    \begin{equation} \label{eq: low deg 1}
    \Pr_{P, x}\left[T[P](x) = Q(x) \land Q(x) \notin \{f_1(x), \ldots, f_k(x) \} \right] \leq \frac{\eps}{100}.
    \end{equation}
    Furthermore, for each $f_i$,
    \begin{equation} \label{eq: low deg 2}
    \Pr_{x}[Q(x) = f_i(x)] \geq \frac{\eps}{1000}.
    \end{equation}
    \end{theorem}
    \begin{proof}
       We take $f_1, \ldots, f_k$ to be all degree $d$ functions that agree with $Q$ in at least $\frac{\eps}{1000}$-fraction of points $x$. By the Johnson bound $k \geq O(\eps^{-2})$. It is clear that each $f_i$ satisfies \eqref{eq: low deg 2}, so it remains to show that \eqref{eq: low deg 1} holds.

       Let $W_i = \{x \in \Ff_q^m \; | \; Q(x) = f_i(x) \}$ and let $W = \cup_{i=1}^k W_i$. Construct the randomized table $Q'$ as follows. For $x \notin W$, set $Q'(x) = Q(x)$. For $x \in W$, set $Q'(x) \in \Ff_q$ uniformly at random. Then by a union bound, with high probability, no degree $d$ function agrees with $Q'$ on more than $\eps/500$-fraction of points. Fix a $Q'$ where this is the case. It follows from Theorem~\ref{thm: basic pvp} that 
       \[
       \Pr_{P, x}\left[T[P](x) = Q'(x) \right] \leq \frac{\eps}{250}.
       \]
       Indeed, if this inequality were false, then Theorem~\ref{thm: basic pvp} would imply that there exists a degree $d$ function agreeing with $Q'$ on $\eps/500$-fraction of points, but no such function exists. To complete the proof, note that if $x \notin W$, then $Q(x) \notin \{f_1(x), \ldots, f_k(x) \}$ and $Q'(x) = Q(x)$. Therefore,
       \[
       \Pr_{P, x}\left[T[P](x) = Q(x) \land Q(x) \notin \{f_1(x), \ldots, f_k(x) \} \right] \leq \Pr_{P, x}\left[T[P](x) = Q'(x) \right] \leq \frac{\eps}{250}
       \]
    \end{proof}

\subsection{Agreement with the Randomized Plane Table}
We will now show the following.
\begin{theorem} \label{thm: agreement with randomized table}
     Let $T$ be a randomized planes table, let $Q$ be a points table, and let the ambient space be $\Ff_q^m$. If 
    \[
    \Pr_{P, x}\left[T[P](x) = Q(x) \right] = \eps \geq \frac{1000d^{10}}{q^{1/10}},
    \]
    then there exists a degree $d$ function $h$ such that
    \[
    \Pr_{P}[T[P] = h|_P] \geq \frac{\eps}{100}.
    \]
\end{theorem}
\begin{proof}
    Suppose 
    \[
    \Pr_{P, x}\left[T[P](x) = Q(x) \right] = \eps \geq \frac{1000d^{10}}{q^{1/10}},
    \]
and let $f_1, \ldots, f_k$ be the degree $d$ functions given by Theorem~\ref{thm: list decoding pvp}. For each $i$, let $W_i = \{x \in \Ff_q^m \; | \; Q(x) = f_i(x) \}$ and let $W = \bigcup_{i=1}^k W_i$. 

For random $T$ and $P$, let $E_i$ be the event that $T[P] = f_i|_P$. Let $E = E_1 \lor \ldots \lor E_k$. Then,

\[
\Pr_{T, P, x}[T[P](x) = Q(x) \land E] + \Pr_{T, P, x}[T[P](x) = Q(x) \land \overline{E}]  = \eps.
\]

We can bound the second probability on the left hand side above:
\begin{align*}
 \Pr_{T, P, x}[T[P](x) = Q(x) \land \overline{E}] &=  \Pr_{T, P, x}[T[P](x) = Q(x) \land \overline{E} \land x \in W] +  \Pr_{T, P, x}[T[P](x) = Q(x) \land \overline{E} \land x \notin W] \\
 &\leq \Pr_{T, P, x}[T[P](x) = Q(x) \land \overline{E} \land x \in W]  + \frac{\eps}{100} \\
 &\leq \Pr_{T, P, x}[T[P](x) \in \{f_1(x), \ldots, f_k(x) \} \land \overline{E}]  + \frac{\eps}{100} \\
 &\leq  \frac{\eps}{100} + \sum_{i=1}^k  \Pr_{T, P, x}[T[P](x) = f_i(x) \; | \; T[P] \neq f_i|_P] \\
 &\leq \frac{\eps}{100} + k \cdot \frac{d}{q} \\
 &\leq \frac{\eps}{99}.
\end{align*}
It follows that 
\[
\Pr_{T, P, x}\left[T[P](x) = Q(x) \land E \land x \in W \right] \geq \frac{9\eps}{10},
\]
and
\begin{align*}
    \sum_{i, j = 1}^k \Pr_{T, P, x}\left[T[P](x) = Q(x) \land T[P] = f_i|_P \land Q(x) = f_j(x) \right]
    &\geq \Pr_{T, P, x}\left[T[P](x) = Q(x) \land E \land x \in W \right] \geq \frac{9\eps}{10}
\end{align*}
Fix $i \neq j$ and consider a term in the summation above. We can bound the term by 
\[
\Pr_{T, P, x}\left[T[P](x) = Q(x) \land T[P] = f_i|_P \land Q(x) = f_j(x) \right] \leq \Pr_{x} \left[f_i(x) = f_j(x) \right] \leq \frac{d}{q}.
\]
It follows that 
\[
\sum_{i=1}^k \Pr_{T, P, x} \left[T[P](x) = Q(x) \land T[P] = f_i|_P \land Q(x) = f_j(x) \right] \geq \frac{9\eps}{10} - \frac{k^2d}{q}.
\]
Suppose $x$ is sampled first, and then $P \ni x$, and finally $T[P]$. We can upper bound  the probabilities in the summation as
\[
\sum_{i = 1}^k \Pr_{x}[x \in W_i] \cdot \Pr_{x \in W_i, P \ni x, T}[T[P] = f_i|_P] = \sum_{i = 1}^k \Pr_{x}[x \in W_i] \E_{x \in W_i, P \ni x}[F_i(P)].
\]
Where, for each $i$, let $F_i : G(m, 2) \xrightarrow{} [0,1]$ be the function given by $F_i[P] = \Pr_{T}[T[P] = f_i|_P]$. Finally, because each $W_i$ consists of at least $\eps/1000$-fraction of points, we have
\[
\left|\E_{P}[F_i(P)] -  \E_{x \in W_i, P \ni x}[F_i(P)]\right| \leq \frac{q^{-1}}{\sqrt{\eps/1000}}
\]
Putting everything together, we get that
\[
\sum_{i = 1}^k \Pr_{x}\left[x \in W_i \right] \E_{P}[F_i(P)] \geq \frac{4\eps}{5}.
\]
It follows that there exists some $i$ such that 
\[
\E_{P}[F_i(P)] \geq \frac{4\eps}{5} \cdot \left(\sum_{i = 1}^k \Pr_{x}\left[x \in W_i \right] \right)^{-1}.
\]
To conclude, note that,
\[
1 \geq \Pr_{x}\left[x \in W \right] \geq \sum_{i = 1}^k \Pr_{x}\left[x \in W_i \right] - \sum_{i \neq j} \Pr_{x} \left[x \in W_i \cap W_j \right].
\]
For fixed, $i \neq j$, $\Pr_{x} \left[x \in W_i \cap W_j \right] \leq \frac{d}{q}$. It follows that,
\[
 \sum_{i = 1}^k \Pr_{x}\left[x \in W_i \right] \leq 1 + \frac{k^2d}{q}.
\]
As a result, for the degree $d$ function $f_i$, we have
\[
\E_{P}[F_i(P)]  = \E_{T, P}[T[P] = f_i|_P] \geq \frac{\eps}{2}.
\]
\end{proof}

\vspace{5cm}

Now let $A(T, P, x)$ be the indicator for the event that $T[P](x) = Q(x) \land E$. Combining the previous two equations, we have
\[
E_{T, P, x}[A(T, P, x)] \geq \frac{98\eps}{99}.
\]
It follows that
\begin{align*}
    \Pr_{T,P_1, x\in P_1, P_2 \ni x}\left[T[P_1](x) = T[P_2](x) \land E(P_1) \land E(P_2) \right] &\geq \E_{x, T} \left[ \E_{P_1, P_2}\left[A(T, P_1, x)A(T, P_2, x) \right] \right] \\
    &= \E_{x,T} \left[ \E_{P_1}\left[A(T, P_1, x) \right]^2\right] \\ 
    &\geq \left( \E_{x,T} \left[ \E_{P_1}\left[A(T, P_1, x)\right]\right]\right)^2 \\
    &\geq \left(\frac{98\eps}{99}\right)^2.
\end{align*}

Thus,

\[
\sum_{i, j} \Pr_{T, P_1, x, P_2}\left[T[P_1](x) = T[P_2](x) \land T[P_1] = f_i|_{P_1} \land T[P_2] = f_j|_{P_2} \right] \geq \left(\frac{98\eps}{99}\right)^2.
\]
Fix $i \neq j$. Then,
\[
\Pr_{T, P_1, x, P_2}\left[T[P_1](x) = T[P_2](x) \land T[P_1] = f_i|_{P_1} \land T[P_2] = f_j|_{P_2} \right] \leq \Pr_x[f_i(x) = f_j(x)] \leq \frac{d}{q}.
\]
It follows that, 
\begin{align*}
\sum_{i} \Pr_{T, P_1, x, P_2}\left[T[P_1](x) = T[P_2](x) \land T[P_1] = f_i|_{P_1} \land T[P_2] = f_i|_{P_2} \right] &= \sum_{i} \Pr_{T, P_1, x, P_2}\left[T[P_1] = f_i|_{P_1} \land T[P_2] = f_i|_{P_2} \right]\\
&\geq \frac{9\eps^2}{10}.
\end{align*}

For each $i$, let $F_i : G(10, 2) \xrightarrow{} [0,1]$ be the function given by $F_i[P] = \Pr_{T}[T[P] = f_i|_P]$. Rewriting the above, we get,
\[
\sum_{i} \langle F_i, \mathcal{A} F_i \rangle \geq \frac{9\eps^2}{10},
\]
where $\mathcal{A}$ is the adjacency operator given by,
\[
\mathcal{A}F(P) = \E_{x \in P, P' \ni x}[F(P')].
\]
Using the fact that the second eigenvalue of $\mathcal{A}$ is $q^{-2}$, we have, 
\[
\sum_{i} \mu(F_i)^2 \geq \frac{8\eps^2}{10}.
\]
Say $\mu(F_1)$ is the largest of $\mu(F_i)$. Then
\[
\mu(F_1)^2 \geq \frac{8\eps^2}{10} \cdot \frac{1}{\sum_{i} \mu(F_i)}
\]
We conclude by giving an upper bound on $\sum_{i} \mu(F_i)$. Let $B_i$ be the event that $T[P] = f_i|_P \land x \in W_i$. The probability that $T$ and $Q$ pass the plane versus point test is at least:

\[
\sum_{i= 1}^k \Pr_{T, x, P}\left[B_i \right] - \sum_{i \neq j} \Pr_{T, x, P}\left[B_i \land B_j\right] \geq \sum_{i= 1}^k \Pr_{T, x, P}\left[B_i \right] - k^2\frac{d}{q},
\]
where we use the fact that for a fixed $i \neq j$, each term in the second summation is at most $\Pr_x[f_i(x) = f_j(x)] \leq d/q$. Moreover, for each $i$, 
\[
\Pr_{T, x, P}\left[B_i \right] = \Pr_{x \in W_i} \cdot \Pr_{T, x\in W_i, P \ni x}[T[P] = f_i|_P] \geq \frac{\eps}{1000} \cdot \E_{x \in W_i, P \ni x}[F_i[P]] \geq \frac{\eps}{1000} \left( \mu(F_i) - q^{-1/2} \right).
\]
It follows that 
\[
\sum_{i=1}^k \mu(F_i) \leq ...
\]


==> rbr_soundness_low_degree.tex <==
\section{Round-by-Round Soundness Proofs}

The main lemmas required for our proof of RBR-soundness are the following low degree testing result. Recall that $S = I_{2,d,4}(\Ff_q)^2$.
\begin{lemma} \label{lem: strong line vs point}
Suppose $f: \Ff_q^m \to \Ff_{q'}$ satisfies $\agr_d(f) \leq \eps \leq \frac{1}{4}$. Then,
\[
\Pr_{L \in \ag(\Ff_q^m, 1)}[\agr_d(f|_L) \geq \frac{1}{2}] \leq O\left(\frac{d}{q} \right)^{\tau}.
\]
\end{lemma}
\begin{proof}
    Deferred to Section ...
\end{proof}

\begin{lemma} \label{lem: strong pvp}
    Suppose $Q: \Ff_q^m \to \Ff_{q'}$ satisfies $\agr_d(Q) \leq \eps$. Then
    \[
    \Pr_{P \subseteq \Ff_q^m}[\agr_d(Q|_P) \geq 1.2\eps] \leq \frac{100}{\eps^2 q},
    \]
    where $P$ is a uniformly random affine plane in $\Ff_q^m$.
\end{lemma}
\begin{proof}
    Deferred to \cref{sec: custom pvp}.
\end{proof}
\begin{lemma} \label{lm: improved pvp fold}
Let $f: \Ff_q^2 \to \Ff_{q'}$ be a function which satisfies $\agr_{5d}(f) \leq \eps$. Then for any $Q: \Ff_q^5 \to \Ff_{q'}$, the following holds. Choose a random tuple $(s_1, a_1, a_2,\ldots, a_5) \in S \times S \times \Ff_q^{2m} \times \cdots \times \Ff_q^{2m}$ and set $M = s_1 + \spa(a_1,\ldots, a_5)$. 

With probability at most $\frac{100}{\eps^2d^{-1/2}}$, there exists a degree $5d^{1/2}$ function $H: \Ff_q^5 \to \Ff_{q'}$ satisfying
\begin{itemize}
    \item $\agr(H, Q|_M) \geq 1.2\eps$,
    \item $H$ agrees with $f$ on at least $1.2 \eps$ of the special points in $M$.
\end{itemize} 
\end{lemma}
\begin{proof}
    Deferred to \cref{sec: low deg manifold}
\end{proof}


\subsection{RBR-Soundness for Weak RM IOPP}
We will show RBR-Soundness for the Weak RM IOPP. This will require us to defined a doomed state after each round of interaction. Recall that we define the initial state as follows.
\begin{state}
    The beginning state is doomed if and only if 
    \[
    \agr_{\overline{d}}(f) \leq \eps,
    \]
    where we $\overline{d} = 2md$.
\end{state}
In the remainder of this subsection we will go through each round of interaction, define the doomed state afterwards, and show soundness for each round.

\subsubsection{Pre-Folding Step:}
\paragraph{First Round of Interaction:}

\begin{itemize}
    \item \textbf{P: } The Prover sends an empty message.
    \item \textbf{V: } The Verifier chooses $T$ random affine planes $P_1, \ldots, P_T \subseteq \Ff_{q}^m$ and samples $\xi_1, \ldots, \xi_T \in \Ff_{q'}$ according to the proximity generator. The Verifier sends each of the planes and coefficients to the Prover.
\end{itemize}
After this round of interaction, the state function is as follows.
\begin{state}
    The state is doomed if and only if,
    \[
    \agr_{\overline{d}}\left(\sum_{i=1}^T \xi_i \cdot f|_{P_i}\right) \leq O(\eps).
    \]
\end{state}
Soundness of this round follows from the following lemma.
\begin{lemma}
    If the previous state was doomed, then the next state is doomed with probability at least $1-2^{-\lambda}$. 
\end{lemma}
\begin{proof}
Suppose the previous state was doomed. Then,
\[
\agr_{\overline{d}}(f) \leq \eps.
\]
 By \cref{lem: strong pvp}, we have
    \[
    \Pr_{P \subseteq \Ff_q^3}[\agr_{\overline{d}}(f|_P) \geq 1.2\eps] \leq \frac{100}{\eps^2 q}. 
    \]
It follows by the choice of $T$ that with probability at least $1 - 2^{-2\lambda}$, there is at least one plane $P_i$ such that 
$\agr_{\overline{d}}(f|_{P_i}) \leq 1.2\eps$. If this is the case, then with probability at least $1 - 2^{-2\lambda}$ we have that
\[
\agr_{\overline{d}}\left(\sum_{i=1}^T \xi_i \cdot f|_{P_i}\right) \leq 4.8\eps,
\]
by \cref{thm: prox gen RM without corr orig}. The lemma follows.
\end{proof}

\paragraph{Second Round of Interaction:} 
\begin{itemize}
    \item \textbf{P: } The Prover sends $g: \Ff_q \to \Ff_{q'}$ where in the honest case,
    \[
    g(x) = \sum_{i = 1}^T \xi_i \cdot f|_{P_i}(x).
    \]
    \item \textbf{V: } The Verifier chooses points $\beta_1, \ldots, \beta_{T}$ uniformly at random checks if:
    \[
    g(\beta_j) = \sum_{i = 1}^T \xi_i \cdot f|_{p_i}(\beta_j), \quad \forall j \in [T].
    \]
    If the equation above does not hold for any $j$ then the Verifier rejects and the protocol terminates.
\end{itemize}
After this round of interaction, the state function is as follows.
\begin{state}
    The state is doomed if and only if one of the following holds:
    \begin{itemize}
        \item One of the Verifier's checks failed and the Verifier rejects. In this case the protocol terminates and every subsequent round is doomed.
        \item $\agr_{\overline(d)} \leq O(\eps)$
    \end{itemize}
\end{state}
Soundness of this round follows from the following lemma.
\begin{lemma}
    If the previous state was doomed, then the next state is doomed with probability at least $1-2^{-\lambda}$. 
\end{lemma}
\begin{proof}
Let $F = \sum_{i=1}^T \xi_i \cdot f|_{P_i}$. Suppose the previous state is doomed. Then $\agr_{\overline{d}}(F) \leq O(\eps)$, and for any $g$ that the prover sends, one of the following must hold
\begin{itemize}
    \item $\dist(g, F) \geq 1 - \Omega(\eps)$.
    \item $\agr_{\overline{d}}(g) \leq O(\eps)$.
\end{itemize}
In the former case, one of the Verifier's equality checks will fail with probability at least $1 - 2^{\lambda}$ and state is doomed. In the latter case, the state is doomed. The soundness of this round follows.
\end{proof}

\subsubsection{Folding Step:}

\paragraph{Interaction 1:} 
\begin{itemize}
\item \textbf{P:} The Prover sends a function $Q: \Ff_{q}^4 \to \Ff_{q'}$. In the honest case,
        \[
        Q \circ I_{2, md, 4}(x) = g(x).
        \]
        Let $S = I_{2, d, 4}(\Ff_q^2)$.
        \item \textbf{V:} The Verifier chooses $2T$ tuples $(s_1, a_1, a_2, a_3, a_4, a_5) \in S \times S \times \Ff_q^{2m} \times \cdots \times \Ff_q^{2m}$. For each $i \in [T]$, let $M_i: \Ff_q^{5} \to \Ff_{q}^{2m}$ be the $5$-dimensional subspace given by:
        \[
        M_i(\alpha_1, \alpha_2, \alpha_3, \alpha_4, \alpha_5) = s_i + \alpha_1 \cdot a_1 + \sum_{j = 2}^5 \alpha_j \cdot a_j.
        \]
        The Verifier sends all $T$ manifolds to the Prover.
\end{itemize}
At the end of this round the state function is as follows.
\begin{state}
    The state is doomed if and only if for at least one $i$, there does not exist a function of degree $4\overline{d}^{1/2}$ that agrees with $Q|_{M_i}$ on at least $1.2\eps$ of the special points.
\end{state}
\begin{lemma}
    If the previous state was doomed then the next state is doomed with probability at least $2^{-\lambda}$.
\end{lemma}
\begin{proof}
    Follows immediately from \cref{lm: improved pvp fold}.
\end{proof}

\paragraph{Interaction 2:} 
\begin{itemize}
    \item \textbf{P:} The Prover sends an empty message.
     \item \textbf{V:} For each $j \in [T]$, the Verifier chooses points $z^{(j)}_1, \ldots, z^{(j)}_{\lambda} \in A$ and sends these to the Prover. For each $i \in [\lambda]$, let 
        $\beta^{(j)}_i= f \circ  I_{2, md, 4}^{-1} \circ M_j(a^{(j)}_i)$.
        
\end{itemize}

After the Verifier sends $M_1, \ldots, M_T$ in the previous round, let $Q_i := Q|_{M_i}$ for each $j \in [T]$. 

The state function is then defined as follows.
\begin{state}
    The state is doomed if and only if for at least on $j \in [T]$, we have,
    \[
    \agr(Q|_i, \RM[5, d' \; | \; \{a^{(j)}_{i} \mapsto \beta^{(j)}_i \}_{i=1}^{\lambda}]) \leq 1.2\eps.
    \]
\end{state}
\begin{lemma}
    If the previous state was doomed, then for any message that the Prover sends, the next state will be doomed with probability at least $1-2^{-\lambda}$ over the Verifier's message.
\end{lemma}
\begin{proof}
    Since the previous round is doomed, there is at least one $j \in [T]$ such that every function of degree $4\overline{d}^{1/2}$ agrees with $Q_i$ on at most $1.2\eps$ of the points in $A\subseteq \Ff_q^5$, where $A$ is as defined in step c.
    
    Let $\List(Q_i)$ be the list of degree $4\overline{d}^{1/2}$ functions that agree with $Q_i$ on at least $1.2\eps$ fraction of points in $\Ff_q^5$. By  \cref{thm: list decoding}, $|\List(Q_i)| \leq O(1/\eps)$. Furthermore, for each $F \in \List(Q_i)$,
    \[
    \Pr_{x \in A}[F(x) = Q_i(x)] \leq 1.2\eps,
    \]
   and
   \[
   \Pr_{a^{(j)}_{1}, \ldots a^{(j)}_{\lambda} \in A}[F(x) = Q_i(x)] \leq (1.2\eps)^{\lambda}.
   \]
   By a union bound, with probability at least, 
   \[
   1 - O(1/\eps)(1.2\eps)^{\lambda} \geq 1 - 2^{-\lambda},
   \]
   we have that no member of $\List(Q_i)$ agrees with $Q_i$ on $a^{(j)}_{1}, \ldots a^{(j)}_{\lambda}$. In this case, the next state is doomed, so we are done.
\end{proof}

\paragraph{Interaction 3}
During this interaction, the parties perform the side condition IOP. 
\begin{itemize}
     \item \textbf{P + V:} For each $i \in [T]$, both Parties run the IOP for RM-codes with Side Conditions, with the following input:
     \begin{itemize}
         \item Functions $Q|_{M_1}, \ldots, Q|_{M_T}$.
         \item For each $j \in [T]$, the side conditions are 
         \[
         \{a^{(j)}_i \mapsto \beta^{(j)}_i \}.
         \]
         \item Degree parameter $d'$.
     \end{itemize}
Let $G_i: \Ff_q^5 \to \Ff_{q'}$ be the output function.
\end{itemize}

At the end of this interaction, the state function is as follows.
\begin{state}
    The state is doomed if and only if $\agr(d') \leq 40 \eps$, or the Verifier has terminated the side condition IOP protocol early. In the latter case, the Verifier terminates the weak low degree IOP early as well.
\end{state}
\begin{lemma}
    If the previous state was doomed, then the next state is doomed with probability at least $1 - 2^{-\lambda}$.
\end{lemma}
\begin{proof}
    This follows from the Round-by-Round soundness in \cref{thm: side cond iop}
\end{proof}

\subsubsection{Inverse Polynomial Rate RM IOP}

\paragraph{Interaction 1}
\begin{itemize}
\item \textbf{P: } The Prover sends an empty mesage.
 \item \textbf{V: } The Verifier chooses $T$ random affine lines $L_1, \ldots, L_T \subseteq \Ff_{q}^m$ and samples $\xi_1, \ldots, \xi_T \in \Ff_{q'}$ according to the proximity generator. The Verifier sends all of the lines and coefficients to the Prover. For each $L_i$, the univariate function $g|_{L_i}: \Ff_q \to \Ff_{q'}$ is given by,
    \[
    G|_{L_i}(\alpha) = G(L_i(\alpha)).
    \]
\end{itemize}

\begin{state}
    The state is doomed if and only if 
    \[
    \agr_{d'}\left(\sum_{i = 1}^T  \xi_i \cdot G|_{L_i}\right) \leq \frac{1}{2}.
    \]
\end{state}
\begin{lemma}
    If the previous state was doomed, then the next state is doomed with probability at least $1 - 2^{-\lambda}$.
\end{lemma}
\begin{proof}
    By \cref{lem: strong line vs point}, 
    \[
    \Pr_{L}[\agr(G|_L) \geq \frac{1}{2}] \leq O\left(\frac{d'}{q} \right)^{\tau},
    \]
    thus, with probability at least, 
    \[
    1 - O\left(\frac{d}{q} \right)^{T \cdot \tau} \geq 1 - 2^{-\lambda - 10},
    \]
    we have that at least one $i$ satisfies, $\agr(G|_L) < \frac{1}{2}$. Suppose this is the case, then, 
    \[
    \Pr_{\xi_i \in \Ff_{q'}}[\agr_{d'}\left(\sum_{i=1}^T \xi_i \cdot G|_{L_i}\right) > \frac{1}{2}] \leq 2^{-\lambda - 10}.
    \]
    The result follows from a union bound.
\end{proof}

The Round-by-Round soundness of the remainder of the protocol follows from the Round-by-Round soundness of STIR.
\newpage


==> singular_values.tex <==
\section{Second Singular Values}
We state and prove results about the second singular values of various bipartite graphs that are needed.

\subsection{Standard Subspace Versus Subspace Graphs}

In this section we discuss some commonly used subspace versus subspace graphs and state their second singular values. We fix some ambient space $\Ff_q^m$ throughout the section and assume that $m \geq 4$.

\begin{definition}
  We let $\ag(\ell, \ell')$ denote the Affine Grassmann Graph on $\ell$-dimensional affine subspaces with intersection size $\ell'$. The vertices are $\ell$-dimensional affine subspaces and two affine subspaces $U_1, U_2 \subseteq \Ff_q^m$ are adjacent if and only if $\dim(U_1, U_2) = \ell'$.  We let $\mc{T}_{\ell, \ell'}$ denote the adjacency operator of this graph.
\end{definition}


\begin{lemma}
  We have for all $\ell' < \ell \leq \frac{m}{2}$, we have 
    \[
    \lambda(\mc{T}_{\ell, \ell'})) \leq (1+o(1)) q^{\ell' - \ell}.
    \]
\end{lemma}

For the remainder of this section, we use $\mc{T}$

\subsection{Special Line versus Points}
Let $q$ be a power of $2$ and let $d$ be a power of $2$ dividing $q$. Recall that $I_{m, d, 2m}: \Ff_{q}^m \to \Ff_{q}^{2m}$ is the curve given by
\[
I_{m, d, 2m}(x_1, \ldots, x_{m}) = (x_{1}^{d^{1/2}}, x_1, \ldots, x_{m}^{d^{1/2}}, x_m).
\]
Let $S = I_{m, d, 2m}(\Ff_q^m)$. Notice that there is a subfield of $\Ff_q$ of size $d^{1/2}$, $\Ff_{d^{1/2}}$.


Consider the following bipartite graph $\mc{G} = G(L, R)$:
\begin{itemize}
    \item The left side, $\mc{L}$, consists of all tuples of points $(s, a_1, a_2, a_3) \in S \times S \times \Ff_q^{2m} \times \Ff_q^{2m}$.
    \item The right side, $\mc{R}$, consists of all points in $\Ff_q^{2m}$.
    \item For each $\alpha_1, \alpha_2, \alpha_3 \in \Ff_q$ with $\alpha_2,\alpha_3 \neq 0$, we add an edge between $(s, a_1, a_2, a_3) \in L$ and $s +\sum_{i=1}^3 \alpha_i a_i \in \Ff_q^{2m}$.
\end{itemize}

\begin{theorem} \label{thm: special line vs point singular val}
    Let $\mc{T}: L_2(\mc{L}) \to L_2(\mc{R})$ denote the adjacency operator associated with the graph $\mc{G}$. Then, the second singular value of $\mc{T}$ satisfies
    \[
    \lambda_2 \leq (1+o(1)) \frac{1}{q^{1/2}}.
    \]
\end{theorem}
\begin{proof}
    We instead bound the second singular value associated with the operator of the two step random walk from $\mc{R}$ to $\mc{L}$ to $\mc{R}$. This operator is $\mc{T}^{*}\mc{T}$. It is clear that $\mc{G}$ is biregular, so let $d_L$ and $d_R$ denote its left and right degrees respectively. 

    For every pair of points $x, x' \in \Ff_q^{2m}$, let $\mc{T}^* \mc{T}(x,x')$ denote the transition probability of going from $x$ to $x'$ in the two step random walk. Then, 
    \begin{align*}  
    \mc{T}^* \mc{T}(x,x') &= \E_{(s, a_1, a_2, a_3) \in \mc{L}}\Pr_{\alpha'_i, \alpha_i \in \Ff_q}\left[\left(s + \sum_{i=1}^3 \alpha_i a_i = x\right) \land \left( s + \sum_{i=1}^3 \alpha'_i a_i = x'\right) \right] \\
    &= \E_{\alpha'_i, \alpha_i \in \Ff_q}\Pr_{(s, a_1, a_2, a_3) \in \mc{L}}\left[\left(s + \sum_{i=1}^3 \alpha_i a_i = x\right) \land \left( s + \sum_{i=1}^3 \alpha'_i a_i = x'\right) \right] \\
    &=  \E_{\alpha'_i, \alpha_i \in \Ff_q}\Pr_{(s, a_1, a_2, a_3) \in \mc{L}}\left[\left(s + \sum_{i=1}^3 \alpha_i a_i = x\right) \land \left( s + \sum_{i=1}^3 \alpha'_i a_i = x'\right) \right]
    \end{align*}
    If $\alpha_2 \alpha'_3 - \alpha_3 \alpha'_2 \neq 0$, then note that the inner probability above is equal for every pair $(x,x') \in \Ff_q^m$. Indeed, in this case, for any choice of $\alpha_1, \alpha'_1 \in \Ff_q$, $s, a_1 \in S$, and any pair $(x,x') \in \Ff_q^m$, one can verify that the system of equations 
    \begin{align*}
        s + \sum_{i=1}^3 \alpha_i a_i &= x \\
        s + \sum_{i=1}^3 \alpha'_i a_i &= x',
    \end{align*}
    has exactly one solution. It follows that we may write,
    \[
    \mc{T}^* \mc{T} = (1-p)J + p\mc{A},
    \]
    where $J$ is the adjacency operator of the complete graph on $\mc{R}$, and 
    \[
    p = \Pr_{\alpha_2, \alpha_3, \alpha'_2, \alpha'_3 \in \Ff_q}[\alpha_2 \alpha'_3 - \alpha_3 \alpha'_2 = 0] \leq \frac{1}{q} + \frac{4}{q^2}.
    \]
    
    To conclude, we analyze the operator $\mc{A}$, and in particular, the distribution of $x'$ obtained by choosing $x \in \Ff_q^{2m}$ uniformly at random and then $x'$ adjacent to $x$ randomly according to adjacency operator $\mc{A}$.
    
    Note that if $\alpha_2 \alpha'_3 - \alpha_3 \alpha'_2 = 0$ and $\alpha_2, \alpha_3 \neq 0$, then there is some nonzero $\gamma \in \Ff_q$ such that $\alpha'_2 = \gamma \cdot \alpha_2$ and $\alpha'_3 = \gamma \cdot \alpha_3$. Therefore if, 
    \begin{equation} \label{eq: adj x}
    s + \alpha1 a_1 + \alpha_2 a_2 + \alpha_3 a_3 = x,
     \end{equation}

    then, $x'$ is distributed according to
    \[
    x + (\gamma-1)(a_2 + a_3),
    \]
    where $\gamma$ is a uniformly random nonzero element of $\Ff_q$. Its not hard to see that $a_2 + a_3$ is uniformly random in $\Ff_q^{2m}$ if we condition on Equation~\eqref{eq: adj x}. Thus, $x'$ is uniformly random in $\Ff_q^{2m}$.
    
   To bound the second eigenvalue of $\mc{T}^*\mc{T}$, note that for any unit norm $F \in L_2(\mc{R})$ satisfying $\E_{R \in \mc{R}}[F(R)] = 0$, we have,
    \begin{align*}
     \norm{\mc{T}^*\mc{T} F} = \norm{(1-p)JF + p \mc{A}F} = \norm{p \mc{A}F} = p \norm{\mc{A}F}.
    \end{align*}
    In the second transition we are using the fact that $JF = 0$ and in the third transition we use the fact that $\mc{A}$ is an adjacency operator and $F$ has norm $1$.

    Finally, we bound $\norm{\mc{A}F}$:
    \begin{align*}
        \norm{\mc{A}F}^2 &= \E_{R \in \mc{R}}[\mc{A}F(R)^2] \\
        &= \E_{R \in \mc{R}} \left[\E_{R' \sim \mc{A}(R, \cdot)} [F(R')]^2\right] \\
        &\leq \E_{R \in \mc{R}} \left[\E_{R' \sim \mc{A}(R, \cdot)} [F(R')^2]\right] \\
        &= \E_{R'}[F(R')^2] \\
        &= 1.
    \end{align*}
    In the last transition we are using the fact that choosing $R \in \mc{R}$ and then $R'$ adjacent to $R$ with probability proportional to $\mc{A}(R, \cdot)$, $R'$ is uniformly random in $\mc{R}$. The result follows.
\end{proof}

\subsection{Manifold versus Points}
Let $q'$ and $q$ both be powers of two such that $F_{q'}$ is a subfield of $F_{q}$. Let $d$ be a power of two. Recall that $I_{m, d, 2m}: \Ff_{q}^m \to \Ff_{q}^{2m}$ is the curve given by
\[
I_{m, d, 2m}(x_1, \ldots, x_{m}) = (x_{1}^{d^{1/2}}, x_1, \ldots, x_m^{d^{1/2}}, x_m).
\]
Let $S = I_{m, d, 2m}(\Ff_q^m)$. Consider the following bipartite graph $\mc{G}_1 = G(L, R)$. 
\begin{itemize}
    \item The left side, $L$, consists of all affine subspaces $M$ of the form
    \[
    M(\alpha_1, \alpha_2, \alpha_3, \alpha_4) = s + \alpha_1 \cdot s' + C(\alpha_2, \alpha_3, \alpha_4),
    \]
    for points $s, s' \in S$ and linear cubes $C \subseteq \Ff_{q_2}^m$.
    \item The right side consists of all affine lines $\ell \subseteq \Ff_q^{2m}$.
    \item For $C \in L$ and an affine line $\ell \in R$, we have $M$ and $z$ are adjacent if and only if there exist $\alpha_1, \alpha_2 \in \Ff_{q}$ such that the plane $M(\alpha_1, \alpha_2, z_1, z_2): \Ff_q^2 \to \Ff_q^{2m}$ contains $\ell$. Put another, way, there must be $\alpha_1, \alpha_2, \beta \in \Ff_q$ such that
    \[
    \ell(t) = M(\alpha_1, \alpha_2, t, \beta t).
    \]
\end{itemize}

\subsection{Special Lines vs Points}

Let $q'$ and $q$ both be powers of $2$ such that $\Ff_{q}$ is a subfield of $\Ff_{q'}$. Consider the following bipartite graph $\mc{G} = G(\mc{L}, \mc{R})$.
\begin{itemize}
    \item The left side $\mc{L}$ consists of the following sets, which are subsets of lines:
    \[
    L'(a,b) = \{a + \alpha \cdot b \; | \;  \alpha \in \Ff_q \}.
    \]
    \item The right side $\mc{R} = \Ff_{q'}^m$.
\end{itemize}

\begin{lemma} \label{lm: singular value special points line}
    Let $\mc{T}: L_2(\mc{L}) \to L_2(\mc{R})$ denote the adjacency operator associated with the graph $\mc{G}$. Then the second singular value of $\mc{T}$ satisfies
    \[
    \lambda _2 \leq  \frac{1}{\sqrt{q}}.
    \]
\end{lemma}
\begin{proof}
    It suffices to bound the second eigenvalue value of $
   \mc{T}\mc{T}^*$ and then take the square root. This operator has the following transition probability for any pair of points $x, y$:
   \[
   \mc{T}\mc{T}^* (x, y) = \E_{\alpha_1, \alpha_2 \in \Ff{q}} \Pr_{a, b \in \Ff_{q'}^m}[a + \alpha_1 b = x \land a + \alpha_2 b = y].
   \]
   Thus, if we condition on $\alpha_1 = \alpha_2$ and $\alpha_1, \alpha_2 \neq 0$, then the transition probabilities are that of the identity operator. On the other hand, if we condition on $\alpha_1 \neq \alpha_2$, then for any pair $x \neq y$, 
   \[
    \Pr_{a, b \in \Ff_{q'}^m}[a + \alpha_1 b = x \land a + \alpha_2 b = y]
   \]
   is the same. Thus, we get,
   \[
   \mc{T} \mc{T}^* = \frac{1}{q} I_{\mc{R}} + \left(1-\frac{1}{q} \right) J', 
   \]
   where $J'$ is the normalized adjacency operator given by $J'(x,x) = 0, \forall x \in \mc{R}$ and $J'(x,y) = \frac{1}{|\mc{R}-1|}, \forall x\neq y$.   It follows that we can write,
    \[
   \mc{T} \mc{T}^* = \left(\frac{1}{q}-p\right) I_{\mc{R}} +  \frac{|\mc{R}|}{|\mc{R}|-1} J = \left(\frac{1}{q}-p\right) I_{\mc{R}} + \frac{q^m}{q^{m}-1} J
   \]
   where $J$ is the uniform adjacency operator and $p = \frac{1}{|\mc{R}|-1}$. Thus, for any $F \in L_2(\mc{R})$ satisfying $\E_{R \in \mc{R}}[F(R)] = 0$ and $\norm{F} = 1$, we have,
   \[
   \norm{ \mc{T} \mc{T}^* F} = \norm{\left(\frac{1}{q}-p \right) F}\leq \frac{1}{q} \norm{ I_{\mc{R}}F} =\frac{1}{q}. 
   \]
   The result follows.
\end{proof}

==> spectral_sampling.tex <==
\section{Spectral Sampling}
We discuss some tools regarding the singular values of adjacency operators that will be useful. Let $\mc{G} = \mc{G}(A, B, E)$ be a (weighted) graph. Let $n_1 = |A|, n_2 = |B|$. Let $L_2(A)$ denote the set of real-valued functions over $A$ (\textcolor{blue}{that are bounded?}), and define $L_2(B)$ similarly. We let $\mathcal{T}: L_2(A) \to L_2(B)$ be the adjacency operator of $\mc{G}$, defined as follows. For a function $F \in L_2(A)$, $\mathcal{T}F \in L_2(B)$ is given by
\[
\mathcal{T}(b) = \E_{a \sim b}[F(v)],
\]
where $a \in A$ is a random neighbor of $b$ sampled according to the edge weights of $\mc{G}$. In this section, we show the following sampling lemma, which is a more general form of the expander mixing lemma. 

\begin{lemma} \label{lm: spectral sampling}
    Let $\mathcal{T}$ be a biregular adjacency operator with second singular value $\lambda$. Let $S \subseteq A$ have fractional size $|S|/|A| = \eps$. Then for any $G \in L_2(B)$ satisfying $0 \leq G(b) \leq 1$ for all $b \in B$, we have
    \[
    \left|\E_{a \in S, b \sim a}[G(b)] - \mu(G)\right| \leq \frac{\lambda}{\sqrt{\eps}}.
    \]
    where $\mu(G) = \E_{b \in B}[G(b)]$.
\end{lemma}

In order to prove \cref{lm: spectral sampling} we first give some background on singular values of operators. Fix an adjacency operator $\mc{T}: L_2(A) \to L_2(B)$. The transpose of $\mathcal{T}$, denoted $\mathcal{T}^{*}: L_2(B) \to L_2(A)$ is given by
\[
\mathcal{T}^* G(a) = \E_{b \sim a}[G(b)],
\]
for some $G: B \to \mathbb{R}$. Composing $\mathcal{T}^*$ and $\mathcal{T}$ we get an operator $\mc{T}^*\mathcal{T}: L_2(A) \to L_2(A)$. Of interest to us will be the singular values of $\mathcal{T}$.

\begin{definition}
 The operator $\mathcal{T}$ has singular value $\lambda$ if and only if there exist functions $F \in L_2(A), G \in L_2(B)$ satisfying,
 \[
 \mc{T} F = \lambda G \quad \text{and} \quad  \mc{T}^* G = \lambda F.
 \]
 We refer to $F$ and $G$ as right and left eigenfunctions $\mc{T}$ respectively with singular value $\lambda$.
\end{definition}
It is well known that $\mathcal{T}$ has $n_1$ singular values $\lambda_1 \geq \cdots \geq \lambda_{n_1}$. Observe that each singular value is also an eigenvalue of $\mc{T}^* \mc{T}$.
\begin{fact}
    If $\lambda$ is a singular value of $\mc{T}$ with right eigenfunction $F$, then $\lambda^2$ is an eigenvalue of $\mc{T}^* \mc{T}$ with eigenfunction $F$:
    \[
    \mc{T}^* \mc{T} F = \lambda^2 F.
    \]
\end{fact}
We equip the space $L_2(A)$ with the inner product $\langle \cdot, \cdot \rangle$ given by
\[
\langle F_1, F_2 \rangle = \E_{a \in A}[F_1(a) \cdot F_2(a)],
\]
for $F_1, F_2 \in L_2(A)$. Also denote the $p$-norm of a function by,
\[
\norm{F}_p = \left(\E_{a \in A}[|F(a)|^p]\right)^{1/p}.
\]
Of special interest is the $2$-norm, which we will often denote without the subscript for convenience. Note that 
\[
\langle F, F \rangle = \norm{F}_2^2.
\] 
An inner product for $L_2(B)$ can be defined similarly and it will always be clear from context which space the inner product is over.

Under this inner product, it is known that both $L_2(A)$ and $L_2(B)$ have orthonormal bases of consisting right and left eigenfunctions of $\mc{T}$ respectively.  
\begin{fact} \label{fact: orthonormal basis}
Let $\lambda_1 \geq \cdots \geq \lambda_{n_1}$ be the singular values of $\mc{T}$. Then there is an orthonormal basis $F_1, \ldots, F_{n_1}$ of $L_2(A)$ and an orthonormal basis $G_1, \ldots, G_{n_2}$ of $L_2(B)$ such that such that each $F_i$ is a right eigenfunction of $\mc{T}$ with singular value $\lambda_i$ and each $G_i$ is a left eigenfunction of $\mc{T}$ with singular value $\lambda_i$. As a consequence,
\[
\langle \mc{T}F_i, G_j \rangle =
\begin{cases}
0 \quad \quad \text{if } i\neq j,\\
\lambda_j G_j \text{ if } $i = j$.\\
\end{cases}
\]
Furthermore, $\lambda_1 = 1$ and $F_1$ and $G_1$ are both the respective all $1$'s function.
\end{fact}
As an immediate consequence of $\cref{fact: orthonormal basis}$ we have the following upper bound on the second singular value of $\mc{T}$. Let $\mathbf{1}$ denote the all ones function.
\begin{lemma}
    Let $\lambda_2$ be the second singular value of $\mc{T}$. Then,
    \[
    \lambda_2 = \max_{F \in L_2(A), \norm{F}_2 = 1, F \perp \mathbf{1}} \norm{\mc{T} F}_2.
    \]
\end{lemma}

Given an $F \in L_2(A)$, it will be convenient to decompose $F$ in terms of its components along the eigenfunctions of $T$ that form an orthoormal basis. We denote the component along the $i+1$th eigenfunction as, $F^{=i}$. More precisely, we have the following.

\begin{definition}
Let $H_i$ be the $i$th right eigenfunction of $\mc{T}$. Then we define $F^{=i} = \inner{F}{H_i} \cdot H_i$.
As a consequence we can write $F = \sum_{i = 0}^{n_1 - 1} F^{=i}$.
\end{definition}
Note that $F^{=0}$ is always a constant function and its norm is the expectation of $F$:
\[
\norm{F^{=0}}_2 = \E_{a \in A}[F(a)].
\]

\begin{definition}
We say that a bipartite graph $\mc{G} = \mc{G}(A,B,E)$ is biregular if the following distributions are uniform over $B$ and $A$ respectively:
\begin{itemize}
    \item Choose $a \in A$ uniformly, and output $b \sim a$,
    \item Choose $b \in B$ uniformly, and output $a \sim b$.
\end{itemize}
\textcolor{red}{The placement of this definition doesn't make any sense.}
\end{definition}
If $\mc{T}$ is the adjacency operator of a biregular graph, then we have,
\[
\inner{F}{G} = \inner{\mc{T}F}{\mc{T}G} = \inner{\mc{T}^*F}{\mc{T}^*G}. 
\]
\textcolor{red}{this equation makes no sense; only one of the last two quantities can make sense, depending on the size $F$ and $G$ are defined on.}
In this case, we refer to $\mc{T}$ as biregular.

We are now ready to show the spectral sampling lemma. It can be thought of as an extension of the expander mixing lemma to the functional setting above.

\begin{proof}[Proof of Lemma~\ref{lm: spectral sampling}]
    Let $F \in L_2(A)$ be the indicator function for $S$. Then we can express 
    \[
    \E_{a \in S, b \sim a}[G(b)] = \frac{\inner{\mc{T}F}{G}}{\eps}.
    \]
    For $i = 0, \ldots, n_1-1$, let $F^{=i}$ denote the part of $F$ along its $i+1$th singular value. Define $G^{=0}, \ldots, G^{=n_2-1}$ similarly. We can decompose, 
    \begin{align*}
        \inner{\mc{T}F}{G} = \left \langle \sum_{i=0}^{n_1-1} \mc{T} F^{=0},\sum_{i=0}^{n_2-1}  G^{=0}\right \rangle
        %= \sum_{i = 0}^{\min(n_1-1, n_2-1)} \langle \mc{T}F^{=i}, G^{=i} \rangle 
        = \eps \mu(G) + \sum_{i = 1}^{\min(n_1-1, n_2-1)} \langle \mc{T}F^{=i}, G^{=i} \rangle.
    \end{align*}
It follows that,
\[
\left |\E_{a \in S, b \sim a}[G(b)]  - \mu(G) \right| \leq \left| \frac{ \sum_{i = 1}^{\min(n_1-1, n_2-1)} \langle \mc{T}F^{=i}, G^{=i}\rangle}{\eps} \right|
\]
To conclude, we bound each term in the numerator. For any $i \geq 1$ we have by Cauchy-Schwarz
\begin{align*}
    \langle \mc{T}F^{=i}, G^{=i} \rangle \leq \norm{\mc{T}F^{=i}}_2\cdot \norm{G^{=i}}_2  
    %\leq \sqrt{\inner{\mc{T}F^{=i}}{\mc{T}F^{=i}}} 
    = \sqrt{\inner{\mc{T}^* \mc{T} F^{=i}}{F^{=i}}}\norm{G^{=i}}
    \leq \lambda \norm{F^{=i}}_2\norm{G^{=i}_2},
\end{align*}
where $\mc{T}^*$ is the adjoint operator of $\mc{T}$. Plugging this in above and using Cauchy-Schwarz again gives
\[
\left |\E_{a \in S, b \sim a}[G(b)]  - \mu(G) \right|
\leq \frac{\lambda}{\eps}
\sum\limits_{i\geq 1}\norm{F^{=i}}_2
\norm{G^{=i}}_2
\leq 
\frac{\lambda}{\eps}
\sqrt{\sum\limits_{i\geq 1}\norm{F^{=i}}_2^2}
\sqrt{\sum\limits_{i\geq 1}\norm{G^{=i}}_2^2},
\]
which is at most $\frac{\lambda}{\eps}\norm{F}\norm{G}\leq \frac{\lambda}{\sqrt{\eps}}$
using $\norm{F}=\sqrt{\eps}$ and $\norm{G}\leq 1$.
\end{proof}

==> subspace_low_degree.tex <==
\section{Subspace Agreement Tests}
In this section we show results related to the Plane versus Point and Line versus Point tests that are necessary for our analysis. Both of these tests are specific cases of subspace agreement tests that are well studied in the PCP literature. 

For our purposes, we require tailored forms of these results that are obtained through straightforward modifications of known results. We derive our tailored results in this section. The following spectral fact will be useful for us. Throughout the section, we fix an ambient space $\Ff_q^m$. For our purposes, one should think of $m = O(1)$.

Let $G_{a, b}$ be the bipartite inclusion graph between $a$-dimensional affine subspaces and $b$-dimensional affine subspaces where $a > b$. That is the graph has parts $\mathcal{A}, \mathcal{B}$ where $A$ consists of all  $a$-dimensional affine subspaces in $\Ff_q^m$ and $\mathcal{B}$ consists of all $b$-dimensional affine subspaces in $\Ff_q^m$. Two vertices $U \in \mc{A}$, $V \in \mc{B}$ are adjacent if $U \supset V$. It is well known that the second singular value of $G_{a,b}$ is $q^{-(a-b)/2}$. By the expander mixing lemma, we get the following convenient sampling lemma.
\begin{lemma} \label{lm: sampling}
   Let $G_{a,b}$ be the bipartite inclusion graph as described above and let $B \subseteq \mc{B}$ and let $\mu(B) = |B|/\mc{B}$. Then for any $A \subseteq \mc{A}$, we have,
   \[
   \left|\Pr_{U \in \mc{A}}[U \in A] - \Pr_{V \in \mc{B}, U \supset V}[U \in A]\right| \leq \frac{q^{-(a-b)/2}}{\sqrt{\mu(B)}}.
   \]
\end{lemma}

The starting point of our results in this section will be the following theorem.


\begin{theorem} \label{thm: line vs point points agree}
There exists a constant $0 < \tau \leq 1/100$ such that the following holds. Suppose $Q: \Ff_q^m \to \Ff_q$ is a points table, suppose $T$ is a lines table assigning each line $L \subseteq \Ff_q^m$ a univariate degree $d$ function from $L \to \Ff_q$, and suppose 
\[
\Pr_{x \in \Ff_q^m, L \ni x}[T[L](x) = Q(x)] \geq \eps.
\]
Then there is a degree $d$ polynomial $F$ satisfying,
\[
\Pr_{x \in \Ff_q^m}[F(x) = Q(x)] \geq \eps - (d/q)^\tau.
\]
\end{theorem}


\input{line_plane/line_vs_point}
%\input{line_plane/plane_vs_point}

==> sumcheck.tex <==
\section{Sumcheck}
In this section we describe our Poly-IOPs for sumcheck. 

\subsection{Univariate}
This is the univariate sumcheck used in STIR.

\subsection{Multivariate 1}
We describe a multivariate sumcheck protocol. This sumcheck protocol is partially compatible with our weak low degree test, as we will see later.

Given as input a function $\widehat{f}: \Ff_{q'}^m \to \Ff_{q'}$, we describe a protocol to verify if
\[
\sum_{a \in H^m} \wh{f}(a) = \beta,
\]
where $\widehat{f}$ has some prescribed degrees $(d, 2d)$. 

\begin{theorem}
    Given a function $\wh{f}: \Ff_{q'}^m \to \Ff{q'}$, there is a sumcheck Poly-IOP with the following properties.

    \begin{itemize}
        \item Query Complexity: $O(1)$.
        \item Round Complexity: $O(1)$.
        \item Number of Distinct Degrees: $O(1)$.
        \item Maximum Degree: $O(d)$.
        \item Completeness: If $\widehat{f}$ has individual degrees $n^{1/m}$ and satisfies
        \[
        \sum_{\vec{a} \in H^m} f(\vec{a}) = \beta,
        \]
        then the honest Prover makes the Verifier accept with probability $1$.
        \item RBR-Soundness: If $\widehat{f}$ has total degree at most $O(mn^{1/m})$, then the protocol has RBR-Soundness $2^{-\lambda}$ where the initial state is doomed if and only if 
        \[
        \sum_{\vec{a} \in H^m} f(\vec{a}) \neq \beta.
        \]
    \end{itemize}
\end{theorem}


\vspace{0.5cm}

We describe the poly-IOP. 

\begin{enumerate}
\item For $i = 1$:
\item \textbf{P:} The Prover sends a polynomial $\wh{F}_1: \Ff_{q'} \to \Ff_{q'}$ with prescribed degrees $(n^{1/m}, n^{1/m})$. In the honest case, $\wh{F}_1$ satisfies,
    \[
    \wh{F}_{1}(x) = \sum_{\vec{b} \in \Ff_{q'}^{m-1}} f( x, \vec{b}).
    \]

\item \textbf{P + V:} Both parties run the univariate sumcheck protocol to check that:
\[
\sum_{\alpha \in H} \wh{F}_1(\alpha) = \beta.
\]
    
\item \textbf{V:} The Verifier chooses $\zeta_1 \in \Ff_{q'}$ uniformly at random.


\item For $i = 2,\ldots, m-1$:
    \item \textbf{P:} The Prover sends a polynomial $\wh{F}_i: \Ff_{q'} \to \Ff_{q'}$ with prescribed degrees $(n^{1/m}, n^{1/m})$. In the honest case, $\wh{F}_i$ satisfies,
    \[
    \wh{F}_{i}(x) = \sum_{\vec{b} \in \Ff_{q'}^{m-i}} f(\zeta_1, \ldots, \zeta_{i-1}, x, \vec{b}).
    \]

\item \textbf{P + V:} Both parties run the univariate sumcheck protocol to check that:
\[\
\sum_{\alpha \in H} \wh{F}_i(\alpha) =  \wh{F}_{i-1}(\zeta_{i-1}).
\]

\item \textbf{V:} The Verifier chooses $\zeta_i \in \Ff_{q'}$ uniformly at random.

\item End For.

\item \textbf{V:} The Verifier chooses $\zeta_m$ uniformly at random and checks if
\[
\wh{F}_{m-1}(\zeta_1, \ldots, \zeta_m) = f(\zeta_1, \ldots, \zeta_m).
\]
\end{enumerate}

\subsection{Completeness}
We show the completeness claim for the sumcheck protocol described. 
\subsection{Round-by-Round Soundness}
Suppose the initial state is doomed. We may assume that $\wh{f}$ has degree at most $O(mn^{1/m})$ and 
\[
\sum_{\vec{a} \in H^m} \wh{f}(\vec{a}) \neq \beta.
\]
We define the state functions for the rest of the protocols and show soundness for each round of interaction.

\paragraph{Interaction 1:} 
\begin{itemize}
   \item \textbf{P:} The Prover sends a polynomial $\wh{F}_i: \Ff_{q'} \to \Ff_{q'}$ with prescribed degrees $(n^{1/m}, n^{1/m})$. In the honest case, $\wh{F}_i$ satisfies,
    \[
    \wh{F}_{i}(x) = \sum_{\vec{b} \in \Ff_{q'}^{m-1}} f( x, \vec{b}).
    \]
    \item \textbf{V:} The Verifier sends an empty message.
\end{itemize}

\begin{state}
    The state is doomed if and only if one of the following holds:
    \begin{itemize}
        \item $\sum_{\alpha \in H} \wh{F}_1(\alpha) \neq \beta$,
        \item $\sum_{\alpha \in H} \wh{F}_1(\alpha) \neq \sum_{\vec{a} \in H^m} f(\vec{a}).$
    \end{itemize}
\end{state}

\begin{lemma}
   If the previous state is doomed, then the next state is doomed with probability $1$. 
\end{lemma}
\begin{proof}
    The proof is immediate.
\end{proof}


\paragraph{Interaction 2:} 
\begin{itemize}
    \item \textbf{P + V:} Both parties run the univariate sumcheck protocol to check that:
    \[
    \sum_{\alpha \in H} \wh{F}_1(\alpha) = \beta.
    \]
\end{itemize}

\begin{state}
    The state is doomed if and only if one of the following holds
    \begin{itemize}
        \item The Verifier rejects during the univariate sumcheck (in which case the protocol has terminated),
        \item $\sum_{\alpha \in H} \wh{F}_1(\alpha) \neq \sum_{\vec{a} \in H^m} f(\vec{a}).$
    \end{itemize}
\end{state}
\begin{lemma}
   If the previous state is doomed, then the next state is doomed with probability at least $1-2^{-\lambda}$. 
\end{lemma}
\begin{proof}
    Assume that the previous state was doomed, then one of the following holds:
    \begin{itemize}
         \item $\sum_{\alpha \in H} \wh{F}_1(\alpha) \neq \beta$,
        \item $\sum_{\alpha \in H} \wh{F}_1(\alpha) \neq \sum_{\vec{a} \in H^m} f(\vec{a}).$
    \end{itemize}

    If the first item holds, then soundness follows from the univariate sumcheck protocol. If the second item holds, then the next state is doomed with probability $1$.
\end{proof}

\paragraph{Interactions during the Loop:} 
\begin{itemize}
    \item \textbf{P:} The Prover sends a polynomial $\wh{F}_i: \Ff_{q'} \to \Ff_{q'}$ with prescribed degrees $(n^{1/m}, n^{1/m})$. In the honest case, $\wh{F}_i$ satisfies,
    \[
    \wh{F}_{i}(x) = \sum_{\vec{b} \in \Ff_{q'}^{m-i}} f(\zeta_1, \ldots, \zeta_{i-1}, x, \vec{b}).
    \]
    \item \textbf{P + V:} Both parties run the univariate sumcheck protocol to check that:
    \[
        \sum_{\alpha \in H} \wh{F}_i(\alpha) =  \wh{F}_{i-1}(\zeta_{i-1}).
\]
\end{itemize}
\begin{state}
    The state is doomed if and only if one of the following holds:
    \begin{itemize}
        \item The Verifier rejects during the univaraite sumcheck, in which case the protocol terminates.
        \item $\sum_{\alpha \in H} \wh{F}_i(\alpha) \neq \wh{F}_{i-1}(\zeta_{i-1})$.
    \end{itemize}
\end{state}
\begin{lemma}
    If the previous state was doomed then the next state is doomed with probability at least $1- 2^{-\lambda}$.
\end{lemma}
\begin{proof}
   If the protocol has already terminated then we are done. Thus, we may assume that 

\end{proof}
% \subsection{Multivariate}
% We give a Poly-IOP for performing sumcheck that utilizes multivariate polynomials. Given as input a function $f: H^m \to \Ff_{q'}$, we describe a protocol to verify if
% \[
% \sum_{a\in H^m} w(a)\cdot f(a) = \alpha,
% \]
% where $w: H^m \to \Ff_{q'}$ is a weight function known to both the Verifier and Prover. 

% \begin{theorem} \label{thm: multi sumcheck}
%     Let $f, w: H^m \to \Ff_{q'}$ be input functions where $H$ is a multiplicative subgroup of the field $\Ff_{q'}$.
    
%     Then there is a Poly-IOP to check if $\sum_{a \in H^m} f(a) \cdot h(a) = \alpha$, in which the Prover sends polynomials from $\Ff_{q'}^m \to \Ff_{q'}$ with the following properties:
%     \begin{itemize}
%         \item Completeness: If $\sum_{a \in H^m} f(a) \cdot w(a) = \alpha$, then there is a Prover strategy which makes the Verifier accept with probability $1$:
%         \item $t(\cdot)$-flexible Soundness: The Poly-IOP has $t(\cdot)$-flexible soundness $t(|H|)/q$ where $t(x) = C x \log (x)$ for some constant $C$.
        
%     \end{itemize}
% \end{theorem}

% Fix $t(x) = Cx\log(x)$ as given in the statement of \cref{thm: multi sumcheck}.
% Let $d = |H|$ and let $\ell = C\log(d)$. Set $d_i = \ell \cdot d - 1$ for each $0 \leq i \leq \ell$. By \cref{lm: primes exist} there exist primes $k = O(\log d)$ prime numbers $p_1, \ldots, p_k$ such that for every $0 < c < d-1$, there is some $p_j$ such that 
% \[
% c \not \equiv p_j \pmod{p_j},
% \]
% and 
% \[
% p_1 \cdots p_k \geq 100d_{\ell}.
% \]

% For each $i \in [k]$, let 
% \[
% \Res_i =\{0,\ldots, d-2\} \setminus \{d_1 \pmod{p_i}, \ldots, d_\ell \pmod{p_i} \}.
% \]
% In words, $\Res_i$ contains every residue modulo $p_i$ except for the residues of $d_1, \ldots, d_{\ell}$. By construction, we have the following fact.

% \begin{fact}
%     For every $c \in \{0,\ldots, d-2\}$, there is some $p_i$ such that the residue of $c$ modulo $p_i$ is in $\Res_i$. Equivalently there is a $p_i$ which does not divide any of $c - d_1, \ldots, c-d_{\ell}$. 
% \end{fact}

% We now describe the multivariate Poly-IOP for sumcheck.

% \newpage

% \noindent \textbf{$m$-variate Sumcheck}
% \begin{enumerate}
%     \item \textbf{P:} The Prover sends polynomials $F_0$ and $\{F_{i,j}\}_{i \in [k], j \in \Res_i}$ such that,
% \begin{align*}
% w(x_1,\ldots, x_m) \cdot f(x_1, \ldots, x_m) &=\frac{\alpha}{|H|} +  V_{H}(x_1,\ldots, x_m) \cdot F_0(x_1,\ldots, x_m) \\
% &+  \sum_{\vec{i} \in [k]^m} \; \sum_{\vec{e} \in \Res_{i_1} \times \cdots \times \Res_{i_m}}x^{\vec{e}} \cdot F_{\vec{i}, \vec{e}}(x_1^{p_{i_1}}, \ldots, x_m^{p_{i_m}}).
% \end{align*}
% Each polynomial has prescribed degree either, $md, md/\log(d), md/\log^2(d)$.


% \item \textbf{V:} The Verifier chooses $\beta\in \Ff^m_{q'}$ and sends it to the Prover. In total, there are $O(\log^{2m}(d))$ terms appearing in the summation above:
% \begin{itemize}
%     \item $-w(\beta) \cdot f(\beta)$,
%     \item $\frac{\alpha}{|H|} + V_H(\beta)F_0(\beta)$
%     \item $\beta^e F_{\vec{i},\vec{e}}(\beta^{p_i}), \quad \forall \vec{i} \in [k]^m, \vec{e} \in \Res_{i_1} \times \cdots \times \Res_{i_m}$.
% \end{itemize}
% Take $H_2$ to be a multiplicative subgroup of $\Ff_{q'}$ such that $|H_2|^m$ is greater than or equal to the number of terms listed above. 

% The Verifier runs another, smaller, sumcheck to check that $\zeta_1 + \zeta_2 + \sum_{i,j} \zeta_{i,j} = 0$.
% \end{enumerate}
